Optimizing Static and Adaptive Probing Schedules for Rapid Event Detection

We formulate and study a fundamental search and detection problem, Schedule Optimization, motivated by a variety of real-world applications, ranging from monitoring content changes on the web, social networks, and user activities to detecting failure on large systems with many individual machines. We consider a large system consists of many nodes, where each node has its own rate of generating new events, or items. A monitoring application can probe a small number of nodes at each step, and our goal is to compute a probing schedule that minimizes the expected number of undiscovered items at the system, or equivalently, minimizes the expected time to discover a new item in the system. We study the Schedule Optimization problem both for deterministic and randomized memoryless algorithms. We provide lower bounds on the cost of an optimal schedule and construct close to optimal schedules with rigorous mathematical guarantees. Finally, we present an adaptive algorithm that starts with no prior information on the system and converges to the optimal memoryless algorithms by adapting to observed data.

==> conclusion.tex <==
\section{Conclusions and Open Problems}
\ahmad{TODO.} s
%Note that storing and/or computing  an optimal, or close to optimal, deterministic schedule can be very expensive. In fact, as in Theorem~\ref{thm:cyclic}, every optimal deterministic schedule is cyclic. However, the the period of the algorithm can be very long, and thus, the algorithm can be very expensive to store or execute. Instead, we show that simple to implement randomized, memoryless schedules provide an efficient alternative to the optimal deterministic schedule.

==> experiment.tex <==
\section{Experimental Results}\label{sec:experiment}

We experimented with four methods for constructing randomized memoryless schedules. Most of our experiments use 1-schedules, and we show later that the results scale to $c$-schedules (see Figure~\ref{fig:scalability}) as expected by the theory.
We use the following 1-schedules:\vspace{-5mm}
\begin{itemize}
\item A uniform schedule  $\R^u = \frac{1}{N}(1,\dots, 1)$.
\item A schedule proportional to the generating probabilities, $\R^{\pi}= \frac{1}{\sum_{i=1}^N \pi_i}(\pi_1,\dots,\pi_N )$.
\item A schedule derived from the first lower bound: $$\R^{\sqrt{}}=\frac{1}{\sum_{i=1}^N \sqrt{\pi_i}}(\sqrt{\pi_1},\dots,\sqrt{\pi_N }).$$
\item A schedule derived from the second lower bound:
$$R^+ =\arg\min_{\mathbf{p}}\paran{\sum_{i=1}^N \frac{(1-\rho_i)\pi_i}{p_i} + \sum_{i=1}^N \frac{\rho_i \pi_i}{\sum_{j=1}^N r_{i,j}p_j}}.$$
\end{itemize}


Our experiments use initial propagation probability $\rho_i =0.95$ for all nodes, and various values of $\phi_i\leq 0.95$, following the intuition that a node is more likely to propagate its own items than others. The results for other initial propagation vectors (< 1) are similar and for lack of space we do not show them here.

When using schedule $\R^{\sqrt{}}$ with initial propagation probabilities $\rho_{i} = 0.95$, the approximation factor guaranteed by Theorem~\ref{cor:randomized_const_approx} is $\frac{1}{0.05} = 20$. However, our experiments show that even this simple method gives very close to optimal schedules. 

All the costs are computed by Monte Carlo method: for each node $i$ with nonzero $\pi_i$, we estimate the expected waiting time of an item generated at $i$, $\omega_i$, by 1000 iterations. We  normalize the generating vector $\pi$ such that $\sum_{i=1}^N \pi_i= 1$. By Equation~(\ref{eq:cost}) this only scales the cost function by $\sum_{i=1}^N \pi_i$.

%The cost of an schedule depends on both topology, and the parameters of the network. In following, we look at 

We experimented with a number of network topologies: we first apply our methods to {\ER} random graphs~\cite{Bollobas200210} with two different densities. These experiments demonstrate the relation
between the topology and the parameters of the problem and the cost of the schedules. Then, we consider social networks, both simulated (Barab\'asi-Albert\cite{BA} and \emph{scale-free}\cite{DirectedScaleFree}) and a real dataset (Facebook~\cite{facebook}).


% We experimented with the following network topologies:
% (i) {\ER} random graphs, (ii) Random graphs \emph{preferential attachment} model\cite{}: Barab\'asi-Albert\cite{} (undirected) and \emph{scale-free}\cite{DirectedScaleFree} (directed), (iii) real social networks: facebook~\cite{}; \ahmad{email communication network of Enron~\cite{}; Twitter?.}, and (iv) examples of bipartite graph that shows how using both the local generating and propagating information helps $\R^+$ to outperform other schedules.



% \subsection{Random Graphs}
\paragraph{{\ER} random graphs}
We considered two examples of {\ER} graphs, $G(n,p)$, with 1000 nodes that pick a an edge with probabilities $0.02$ or $0.1$. In both graphs we assumed the generating vector is uniform and computed the cost of our schedules when all the propagation probabilities are $0.5$, $0.9$, or $0.1$. Note that smaller value of $\phi$ will diminish the  utility of the edges and pushes the graph to the network of  isolated nodes. The costs are summarized in Table~\ref{table:GPM}. Note that here the three schedules $\R^{\sqrt{}}, \R^{\pi}$, and $\R^u$ are equivalent and have the same cost. However, because of the symmetry in $G(n,p)$ graphs and uniformity of both $\pi$ and $\phi$, all the schedules perform very similarly. 


\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\bf cost}   &   \multicolumn{3}{|c|}{$G(1000,0.02)$}   & \multicolumn{3}{|c|}{$G(1000,0.1)$} \\
~ 	&	 $\phi=0.5$& $\phi=0.9$ & $\phi=1$ &$\phi=0.5$& $\phi=0.9$ & $\phi=1$
\\ \hline\hline 
Lower Bound & 50.79 & 50.79  & 50.79 & 50.922 & 50.922 & 50.922  \\ \hline 
$\R^+$ & 53.73 & 53.22  & 53.24 & 52.55 & 52.79 & 52.78  \\ \hline 
$\R^{\sqrt{}},\R^\pi,\R^u$ & 53.54 &  53.45 & 53.35 & 52.71 & 52.59 & 52.72  \\ \hline 
\end{tabular}
}
\caption{The lower bounds and costs of $\R^+, \R^{\sqrt{}}, \R^\pi,$ and $\R^u$.}
\label{table:GPM}
\end{table}



% \subsection{Social Graphs}
\paragraph{Social Networks}
We generated undirected and directed random graphs using the preferential attachment model. 
Since these models do not capture all properties of the social networks (see e.g. \cite{Kronocker_Graph}), we also experimented with a real datasets 
from Facebook which is obtained by combining ego-graphs~\cite{facebook}.

% but they give us some intuitions that help us later for real social networks. We also run our schedules on real datasets as well; facebook, email-Enron.


We estimated the generating and propagation probability of each node as a function of the number of its friends (or followers). Specifically, we used $\pi_i \propto \sqrt{|N(i)|}$, as in~\cite[Fig.~6]{HodasLerman13}, and $\phi_i = \frac{0.22\cdot |N(i)|^{0.21}}{|N(i)|+0.53}$ ~\cite{Hodas12socialcom}. Note that $\phi_i$ is the probability of propagation of other nodes' items, and is a decreasing function on positive integers. Also, since $\rho_i = 0.95$, $1\leq i \leq N$, among the large degree nodes, we expect the \emph{star-shape} propagation pattern for an item: this is because with high probability a generated item will be propagated to the neighbors, and if the degree of the neighbors are large they have small $\phi_i$, and thus, the item has a much smaller chance of being repropagated. A similar observation has been reported in~\cite{Leskovec2007cascadeBlog}.


Our first undirected, simulated graphs are Barab\'asi-Albert (BA) graphs: BA($m$) is BA graph on 1000 nodes, and $m$ edges are attached to each new node (while generating the graph). Figure~\ref{fig:BA} shows the cost of different schedules and the lower bound on the optimal cost. In this experiment, $\R^+$ is consistently the best schedule and its cost is  close to the lower bound. Also, note that in the worst case, $\cost{\R^+}$ and $\cost{\R^{\sqrt{}}}$ are within  1.2146 and  1.4297 factor of the lower bound, respectively (which is much smaller than the guaranteed 20 approximation factor).
In Figure~\ref{fig:BA} the overall cost of BA$(m)$ decreases, since the graphs get denser and an item reaches a larger population when it propagates, and has a higher chance of being detected.

\begin{figure}[h!]
  \centering    
      \includegraphics[width=0.4\textwidth]{Figures/BA.pdf}
  \caption{Cost of the schedules on Barab\'asi-Albert graphs.}
  \label{fig:BA}
\end{figure}


For the directed graphs, we used 8 samples of directed scale-free graphs~\cite{DirectedScaleFree}. We set the parameters as following:
$\alpha=0.41$, $\beta=0.54$, $\gamma=0.05$, $\delta_{\text{in}}=0.2$, $\delta_{\text{out}}=0$,
where $\alpha$ is the probability of adding a new node and link it to via an edge to a previous node according to the $\text{in-degree} + \delta_{\text{in}}$; $\beta$ is the probability of adding an edge $vw$ for two existing nodes, $v$ and $w$, that are chosen independently according to $\text{out-degree} + \delta_{\text{out}}$ and $\text{in-degree} + \delta_{\text{in}}$; $\gamma$ is the probability of linking an existing node chosen according to $\text{out-degree} + \delta_{\text{out}}$ to a new node.
We also remove all the parallel and self-loop edges. The cost of our schedules are presented in Figure~\ref{SF}. Again, consistently $\R^+$ was the best schedule and in the worst case, the costs of $\R^+$ and $\R^{\sqrt{}}$ are within 1.0743 and 1.2209 factor of the lower bound.

\begin{figure}[h!]
  \centering    
      \includegraphics[width=0.4\textwidth]{Figures/SF.pdf}
  \caption{Cost of schedules on directed scale-free graphs.}
  \label{SF}
\end{figure}

Finally, for the real data we used a Facebook dataset (undirected, 4039 nodes -- obtained by combining ego-graphs)~\cite{facebook}.
The results are presented in Fig~\ref{fig:facebook}
Here, similar to our previous observation $\R^+$ (and next $\R^{\sqrt{}}$) outperform other schedules: $\R^+$ is within $1.01$ factor of the lower bound (very close to optimal) and $\R^{\sqrt{}}$ is in $1.29$ factor of the lower bound, and compared to the guaranteed 20 approximation factor, this shows that our schedules are very close to optimal schedules in practice.
% Another important observation is $R^{\sqrt{}}$ is a very easy to compute schedule that can be obtained very fast for much larger graphs.
\begin{figure}[h!]
  \centering    
      \includegraphics[width=0.4\textwidth]{Figures/facebook.pdf}
  \caption{Cost of schedules on Facebook data.}
  \label{fig:facebook}
\end{figure}


% \begin{table}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% 
% {\bf cost} &	 Lower Bound & $\R^+$ & $\R^{\sqrt{}}$ & $\R^\pi$& $\R^u$
% \\ \hline\hline 
% facebook & 239.3 & 242.57& 309.47 &	312.63&	334.40 \\ \hline
% wiki-Vote &  &   & 243.83 & 280.49 &  572.53  \\ \hline 
% % twitter &  &   &  &  &   \\ \hline 
% \end{tabular}
% }
% \caption{Cost of schedules on real datasets.}
% \label{table:real}
% \end{table}

\paragraph{Scaling the cost by $c$-schedules}
We proved for the case of isolated nodes that the cost of the optimal $c$-schedule decreases almost  linearly with $1/c$. Our experiments demonstrate similar relation for the network case. With the exception of some artificial examples, the probability that a 1-schedule probes a node at any given step
is decreasing as the number of nodes increases. 
Thus, if $p_i$ is the probability of probing node $i$ in a 1-schedule, the probability of probing $i$ in a given step of the related $c$-schedule, for $c=o(n),$ is $cp_i\approx 1-(1-p_i)^c$. So, if we obtain a $c$-schedule by running $c$ independent 1-schedule, the cost of the new schedule is almost $\frac{1}{c}$ of 1-schedule's. In Figure~\ref{fig:scalability} we considered the graph BA(1) above, and the $c$-schedules obtained from $\R^+, \R^{\sqrt{}}, \R^{\pi}$, and $\R^u$. As shown, the cost of the schedules scale down by the factor $c$.


\begin{figure}[h!]
  \centering    
      \includegraphics[width=0.5\textwidth]{Figures/scaling.pdf}
  \caption{The cost of $c$-schedules obtained from $\R^+, \R^{\sqrt{}}, \R^{\pi}$, and $\R^u$ on BA(1).}
  \label{fig:scalability}
\end{figure}










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Unknown    Topology  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Unknown topology -- parameters etc}
%As we saw in Section~\ref{sec:experiment} in social networks, the random schedule $\R = R(\mathbf{p})$ where $p_i \propto \sqrt{\pi_i}$ is a very good approximate of an optimal randomized schedule. In this section we present how in some networks we can apply $\R$ just by using local information about the Network. Here we assume that we cannot load the whole network graph in memory, but ego graphs are small enough that fit into in the memory.
%
%The idea is to run a Metropolis-Hastings sampling from the network: we assume that in one step we can query as many nodes their ``number of items'' and crawl the web long enough, but we are allowed to probe only one node. \ahmad{[Conductance of graph!? How fast it converge?]}. So, for a long enough and fixed length $L$ we run a random walk on the network of length $L$ and sample the final node to probe. Note that in this setting, at each step we only use the local information: the neighbors of a node and their number of items. Also, note that we do not use propagation probabilities, and the generating or the edges of the graph may change over the time; as long as these changes are \ahmad{(slow enough)} The algorithm adopts itself. Algorithm~\ref{alg:random-walk} summarize the idea.
%
%
%\begin{algorithm}[htbp] 
%\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%%\DontPrintSemicolon 
%\Input{The node sampled at time $t$, $n(t)$, and the length of the random walk $L$.}
%\Output{$n(t+1)$: The node to be sampled at time $t+1$.} 
%\BlankLine
%\Begin{	
%  \texttt{curr\_node} $\leftarrow n(t)$\;
%  \For{$i\in\set{1,\ldots,L}$}{ 	  
%  }
%}
%\caption{\texttt{Adaptive Sampling}}\label{alg:propagate}
%\end{algorithm}
%
%
%
%




==> graphs.tex <==
\section{General Networks with Propegation}\label{sec:graphs}
Given a network topology and parameters, the problem of finding an optimal $c$-schedule for this input is NP-hard (the related decision problem is NP-complete, see Appendix~\ref{NP-hard}).
We are therefore interested in solutions that are easy to compute and give good approximation. As in our approach to the isolated nodes case we start by proving lower bounds on the optimal cost as a function of the problem's parameters. We then optimize with respect to the lower bounds functions to construct randomized, memoryless schedules. To keep the optimization process tractable we use lower bound functions that are not tight, and therefore,
the algorithms we construct are not optimal. However, we show both analytically and by extensive simulations that our solutions gives close to optimal schedules for a wide variety of practical configurations.

%Building on our solutions for the isolated nodes case, we construct a near optimal randomized, memoryless solution for the general network case.
%We first prove a lower bound on the cost of a randomized memoryless schedule for a network $G$, with generating probabilities vector $\pi$ and propagation vector $\rho$. We then use the lower bound function to obtain an efficient schedule. \ahmad{But this is as good as sqrt method, which is cheaper to compute and can work on evolving graphs.}

%We first compute for any pair of nodes $i,j$, the probability $r_{i,j}$ that an item generated at $i$ reaches node $j$ by the time of that the item stopped propagating to new nodes.



%\paragraph{Notations}
%For a node $i\in\set{1,\ldots,N}$, let 
%\begin{itemize}
% \item $\rho_i$: the probability of propagation at $i$,
% \item $N(i)$: the set of $i$'s neighbors,
% \item $\pi_i$: the probability that $i$ generates a rumor,
% \item $\rho_i$: the probability that $i$ posts a rumor,
% \item $s_{i,j}$: the probability that a rumor generated at $i$ will reach node $j$ in finite time (without any probing --- just the diffusion). So, for example, $s_{i,i} = 1$ and $_{i,j} < 1$ if $i\neq j$.
% \item $s'_{i,j}$: the probability that a rumor (generated at $i$) which is already reached $, reaches to node $j$. Note that if $j\in \set{i} \cup N(i)$ then $s'_{i,j}=1$.
%\end{itemize}

%\paragraph{Schedules} 
%
%\noindent The schedules that we consider are the followings:
%\begin{itemize}
% \item[(i)] $P_{\texttt{unif}}$ which probes each node uniformly at random.
% \item[(ii)] $P_{\sim}$ which probes node $i$ with probability $P_{\sim}(i) ~ \pi_i$.
% \item[(iii)] $P_{\sqrt{~}}$ which probes node $i$ with probability $P_{\sqrt{~}}(i)\sim \sqrt{\pi_i}$: note that $P_{\sqrt{~}}$ is optimal solution for 
% $$\texttt{ minimize }\sum_{i=1}^N \frac{\pi_i}{p_i}.$$
%
% \item[(iv)] $P_1$ which is an optimal solution for  the following optimization:
% $$\texttt{minimize }\sum_{i=1}^N \frac{\pi_i}{\sum_{k=1}^N s_{i,k}p_k}.$$
% 
% \item[(v)] $P_2$ which is an optimal solution for  the following optimization:
% $$\texttt{minimize }\cdot\sum_{i=1}^N (1-\rho_i)\frac{\pi_i}{p_i} + \sum_{i=1}^N \rho_i\frac{\pi_i}{\sum_{k=1}^N s_{i,k}p_k}.$$
% 
% \item[(vi)] $P_3$ which is an optimal solution for  the following optimization:
% $$\texttt{minimize }\sum_{i=1}^N (1-\rho_i) \frac{\pi_i}{p_i} + 
%  \sum_{i=1}^N (1-\rho_i)\rho_i \frac{\pi_i}{\sum_{j\in N(i)}p_j}
% +\cdot\sum_{i=1}^N \rho_i^2\frac{\pi_i}{\sum_{k=1}^N s_{i,k}p_k}.$$
% 
%\item[(vii)] \ahmad{$P_4$ which is an optimal solution for the following optimization:
% $$\texttt{minimize }\sum_{i=1}^N (1-\rho_i) \frac{\pi_i}{p_i} + \sum_{i=1}^N \rho_i\frac{\pi_i}{\sum_{k=1}^N s'_{i,k}p_k}.$$
% $\rightarrow$ This schedule always gives the minimum cost among these schedules.}
% \end{itemize}
%After obtaining all these schedules, we compute their cost through simulations.
%
%\paragraph{Lower Bounds on optimal cost}
%\ahmad{The optimal cost in (vii) is a lower bound: This is because with probability $1-\rho_i$ a rumor will stay at node $i$, so the waiting time is $\frac{1}{p_i}$, or it gets propagated by $i$ with probability $\rho_i$. In the latter case all nodes in $\set{i}\cup N(i)$ will have the rumor. Now by assuming that the rumor will find its final spot immediately, the waiting time is at most $\frac{1}{\sum_j s'_{i,j}p_j}$.}
%
%% First note that the \emph{optimal value} in case (iii) above gives a lower bound on the optimal cost, since we assume that when a rumors comes to system it finds its final spot immediately. Lets denote the optimal value of (iii) by $\ell_1$. Also, we know the expected number of rumors that stays at node $i$ at each time step is $(1-\rho)$. This gives us the second lower bound:
%% $$\ell_2 = (1-\rho)\paran{\sum_{i=1}^N \sqrt{\pi_i}}^2.$$
%% The lower bound that we consider is 
%% $$\text{Our lower bound: } \max\set{\ell_1, \ell_2}$$
%
%
%
%
%
%
%
%
%
%In this section we assume $G=(V,E)$ is the graph of our network. We show when $\rho < 1$ there is always approximation schedules , deterministic and randomized, with constant factor. Then, we study the cases when $\rho=1$ (which is not a realistic assumption). We first show that if the diameter of the graph is bounded, which is a reasonable assumption on social networks, then there are approximation schedules, deterministic and randomized, with constant factor. Next, yet assuming $\rho=1$, we ask the following question: can we obtain \ahmad{non-trivial} approximation schedules by using more detectors? We show that the answer to this question is positive. Specifically,  we can obtain an approximation schedule of factor $O\paran{\log(N) + \frac{1}{1-\delta}}$ by using $O(\log(N)\log(\log(N)))$ detectors, where $0 < \delta < 1$.

\subsection{Lower Bounds}
%We start this section by two lower bounds on the optimal cost (deterministic and randomized), and provide some approximation schedules. Denote $\rho_{\max} = \max\set{\rho_1,\ldots,\rho_N}$ and $\rho_{\min} = \min\set{\rho_1,\ldots,\rho_N}$.
%\begin{theorem}\label{thm:lower_bound_optimal_general_graph:deterministic}
%The cost of a deterministic optimal schedule is at least 
%$\frac{1-\rho_{\max}}{2}\paran{\sum_{i=1}^N \sqrt{\pi_i}}^2 +  \rho_{\min}\paran{\sum_{i=1}^N \pi_i}$.
%\end{theorem}
%
%\begin{proof}
%Obviously, by adding new edges to $G$, the graph of the network, the optimal cost does not increase. So assume $G$ is a complete graph. Also we consider the following relaxing assumption:
%all the propagations of of a generated item happen in one step.
%
%Let $A$ be the set of items that stay at their origin node, and $B$ be the set of items that get shared among all the nodes ($G$ is complete). So, detecting the items in $A$ is similar to the case of $N$ isolated nodes that each node generates a rumor with probability $(1-\rho_i)\pi_i \geq (1-\rho_{\max})\pi_i$, and by Theorem~\ref{thm:lower_bound_optimal} we obtain the first term.
%
%Since $G$ is complete, and we assume all the propagations occur in one step, by probing any node at any step all the items in $B$ are detected. And since the expected number of items in $B$ that are generated at $i$ in any step is $\rho_i\pi_i \geq \rho_{\min}\pi_i$ we get the second term of the lower bound.
%% 
%% So, since $G$ is a complete graph, if an item in $B$ is generated all the nodes will have it. So, catching rumors in $B$ is like having a system that generates $\rho \sum_{i=1}^N \pi_i$ rumors at each time, in expectation, and we serve them all in only one time step. However, catching the rumors of $A$ is similar to catching the rumors in a system of $N$ isolated nodes in which the node $i$ generates a rumor with probability $(1-\rho)\pi_i$. Therefore, by Theorem~\ref{thm:lower_bound_optimal} the optimal cost is at least
%% $$
%% \frac{1-\rho}{2}\paran{\sum_{i=1}^N \sqrt{\pi_i}}^2 +  \rho\paran{\sum_{i=1}^N \pi_i}.
%% $$
%\end{proof}
%


\begin{theorem}\label{thm:lower_bound_optimal_general_graph:randomized}
Let $\R=\mathbf{p}^*$ be an optimal randomized, memoryless 1-schedule for a network $G$ with generating probabilities $\pi$ and propagation vectors $\rho$ and $\phi$. Then $cost(\R)$ is at least
\begin{itemize}[noitemsep,nolistsep]\vspace{-3mm}
\item[{(i)}] $\min_{\mathbf{p}}\sum_{i=1}^N \frac{(1-\rho_i)\pi_i}{p_i}
%=\min_{\mathbf{p}} f_1 (\mathbf{p})
= \paran{\sum_{i=1}^N (\sqrt{(1-\rho_i)\pi_i}}^2$.
%\item[\ahmad{(ii)}]
%$\min_{\mathbf{p}} \sum_{i=1}^N \frac{\pi_i}{\sum_{j=1}^N q_{i,j}p_j}.$
%%=\min_{\mathbf{p}} f_2 (\mathbf{p}),$
%where  $q_{i,j}$ is the probability that an item generated at node $i$ reaches node $j$ %\ahmad{(propagated at once).}
\item[(ii)]
$\min_{\mathbf{p}} \paran{\sum_{i=1}^N \frac{(1-\rho_i)\pi_i}{p_i} + \frac{\rho_i \pi_i}{\sum_{j=1}^N r_{i,j}p_j}},$
%=\min_{\mathbf{p}} f(\mathbf{p}),$
where  $r_{i,j}$ is the probability that an item generated at node $i$ reaches node $j$, conditioned on reaching the neighbors of $i$ (propagated at least once)%\ahmad{(propagated at once)}.
\end{itemize}
\end{theorem}

\begin{proof}
(i) At each step, node $i$ generates with probability $(1-\rho_i)\pi_i$ an item which is not propagated. Optimizing $\mathbf{p}$ for detecting these items (applying Theorem~\ref{thm:lower_bound_optimal}) gives the bound.

(ii) % Here we assume that all propagations of a generated item happen in one step. Note that this by this assumption, we do not increase the cost of the optimal schedule. 
Consider an item generated at node $i$. With probability $\rho_i$ the item is propagated to the neighbors of $i$.
Let $S^i$ be a the set of nodes that received this item by the time it stopped propagating to new nodes, conditioned on the item propagated 
to the neighbors of $i$. Let $S^i_1, \dots, S^i_{2^N}$ be all possible different values of $S^i$ (subsets of $V$), and define $s^i_k=Pr(S^i=S^i_k)$. Note that $\sum_{k=1}^{2^N} s^i_k =1$. 
The expected time to discover an item that reaches a set $S^i_k$, ignoring the time that it took the item to reach all the nodes in that set, is 
$\frac{1}{\sum_{j\in S^i_k} p_j}$. Thus, the expected time to discover an item generated at $i$ is at least
$\sum_{k=1}^{2^N} \frac{s^i_k}{\sum_{j\in S^i_k}p_j}$. Applying Jensen's Inequality~\cite{Cvetkovski201201} (by convexity of the function $f(x)=1/x$) we have
%Applying Cauchy-Schwarz inequality we have 
%$$(\sum_{k=1}^m \frac{s_k}{\sum_{j\in S_k}P_j} )(\sum_{k=1}^m s_k \sum_{j\in S_k} P_j )\geq (\sum_{k=1}^m  s_k)^2 =1.$$
%Thus,
% Applying Jensen's Inequality~\cite{} (since the function $1/x$ is convex) we have
% \begin{align*}
%\sum_{k=1}^m \frac{s_k}{\sum_{j\in S_k}p_j} &\geq \frac{1}{\sum_{k=1}^m s_k \sum_{j\in S_k} p_j }= 
%\frac{1}{\sum_{j=1}^N p_j \sum_{k:j\in S_k} s_k} \\
%&=
%\frac{1}{\sum_{j=1}^N q_{i,j}p_j}.
%\end{align*}

 \begin{align*}
\sum_{k=1}^{2^N} \frac{s^i_k}{\sum_{j\in S^i_k}p_j} &\geq \paran{{\sum_{k=1}^{2^N} s^i_k \sum_{j\in S^i_k} p_j }}^{-1}= 
\paran{{\sum_{j=1}^N p_j \sum_{k:j\in S^i_k} s^i_k}}^{-1}\\
&=
\frac{1}{\sum_{j=1}^N r_{i,j}p_j}.
\end{align*}
Summing over all nodes we obtain the second lower bound. 
%(iii) The third bound is obtained by applying the method of the first bound to items that were not propagated at all, and applying the method of the second bound to items that were propagated at least once.
%%We use a combination of previous two bounds: when an item is generated at node $i$ (a) it stays at $i$ with probability $1-\rho_i$ and then takes on average $1/p_i$ steps to get detected, or (b) it propagates at least once with probability $\rho_i$ and takes one average (at most) $\frac{1}{\sum_{j=1}^N r_{i,j}p_j}$  steps to get detected: we apply the same argument as in part (ii) except that $S$ is restricted only to $S_i$'s that contain $\set{i}\cup N(i)$, which is the 1-neighborhood of $i$.
\end{proof}

Note that the using Jensen's inequality in the proof we replace a sum over exponential number of terms by a sum over a linear number of terms. Thus, we obtain a lower bound expression that we can use in constructing an algorithm for the problem.
%\ahmad{It is easy to see that the third lower bound in Theorem~\ref{thm:lower_bound_optimal_general_graph:randomized} is the better than others. However, the computational cost of each of them is different. In Section~\ref{sec:experiment} we show that in practice these lower bounds are very close, and we can approximate the third bound by the first one. Note that for the first bound we do not need to know anything about the topology of the graph.}



\subsection{Efficient Network Schedules}

We first show that in bounded propagation configurations the isolated nodes schedules gives a constant approximation to the optimal solution. This simple observation is confirmed by many of our simulation results in which the cost of this algorithm is closed to optimal (see Section~\ref{sec:experiment}).\vspace{-5mm}


% Theorem~\ref{thm:lower_bound_optimal_general_graph:deterministic}, we have the following immediate corollary, which states the same non-adaptive randomized algorithm for when the network consists of isolated nodes,  still gives us a constant approximation if $\rho_{\max} < 1$.

\begin{theorem}\label{cor:randomized_const_approx}
Suppose $\rho_{\max} = \max\set{\rho_1,\ldots,\rho_N}< 1$, and $\R = \mathbf{p}$ is a randomized 1-schedule in which $p_i \propto \sqrt{\pi_i}$. Then, $\R$ is a $\frac{1}{1-\rho_{\max}}$-approximation randomized memoryless schedule.
\end{theorem}
\begin{proof}
Let $\O$ be an optimal randomized memoryless 1-schedule then using the first bound in Theorem~\ref{thm:lower_bound_optimal_general_graph:randomized}, \\
$cost(\O)\geq\paran{\sum_{i=1}^N \sqrt{(1-\rho_i)\pi_i}}^2\geq (1-\rho_{\max}) \paran{\sum_{i=1}^N \sqrt{\pi_i}}^2$.
By Theorem~\ref{thm:randomized_schedule}  $\cost{\R} \leq \paran{\sum_{i=1}^N \sqrt{\pi_i}}^2$. Thus,
\begin{align}\label{eq:const_small_rho}
\frac{\cost{\R}}{\cost{\O}} 
&\leq 
\frac{\paran{\sum_{i=1}^N \sqrt{\pi_i}}^2}{{(1-\rho_{\max}})\paran{\sum_{i=1}^N \sqrt{\pi_i}}^2 }  =
\frac{1}{1-\rho_{\max}}, \nonumber
\end{align}
\end{proof}
%Note that if $\rho=1$, then $\cost{\R}/\cost{\O}$ in Equation~(\ref{eq:const_small_rho}) can be as large as $O(N)$, e.g., if $\pi_1=\pi_2=\ldots=\pi_N$. \ahmad{Also, note that one can obtain a deterministic schedule from  the randomized schedule in Corollary~\ref{cor:randomized_const_approx} and obtain a $\frac{2}{1-\rho_{\max}}$-approximation by the method introduced in Section~\ref{sec:approx}}.

Next we use the distributions that minimizes the bound (ii) in Theorem~\ref{thm:lower_bound_optimal_general_graph:randomized} as a randomized memoryless 1-schedules. Let
$$f(\mathbf{p})=f(p_1,\dots,p_N)=\sum_{i=1}^N \frac{(1-\rho_i)\pi_i}{p_i} + \sum_{i=1}^N \frac{\rho_i \pi_i}{\sum_{j=1}^N r_{i,j}p_j}.$$
We first show that the distribution $p^*=\arg\min_{\mathbf{p}} f(\mathbf{p})$
can be computed efficiently, and then discuss the performance of the algorithm.
%
\paragraph{Computation} The matrix  $R=(r_{i,j})$ of the probabilities $r_{i,j}$ can be estimated by Monte Carlo simulations or by algorithm \texttt{Propagate} (Algorithm~\ref{alg:propagate}): where $r_{i,j}^t$ is an estimate of $r_{i,j}$ after $t$ iterations, and $\nu_{i,j}^t$ is an estimate of the probability that an item generated at $i$ reaches $j$ exactly after $t$ step. 


% We now use the \ahmad{third} lower bound function as the base for efficient algorithm that construct randomized probing schedules for general networks. Although we optimize the schedules with respect to a lower bounds that are not always tight, we present extensive simulation results demonstrating the near optimality of our algorithm in a variety of networks and parameters.

% First we need to compute the 
% matrices $S = (s_{i,j})$ and $R=(r_{i,j})$ of the probabilities $r_{i,j}$ that an item that is generated at node $i$ reaches node $j$, and
% the probabilities $r'_{i,j}$  that an item that is generated at node $i$ reaches node $j$ conditioning on the item propagated at least one. These matrices can be estimated by Monte Carlo simulations or compute by algorithm \texttt{Propagate} (Algorithm~\ref{alg:propagate}).

\begin{algorithm}[htbp] 
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%\DontPrintSemicolon 
\Input{The adjacency matrix of the network, $A$, the secondary propagation vector $\phi$, and the number of iterations, $T$.}
\Output{The matrix $R$} 
\BlankLine
\Begin{	
	\For{$i,j\in\set{1,\ldots,N}$}{ 	  
	   \If{$j \in \set{i}\cup N(i)$}{
		$r^0_{i,j}, \nu^0_{i,j}\leftarrow 1$\;
	   } \Else{
	      $r^0_{i,j}, \nu^0_{i,j}\leftarrow 0$\;
	   }
	  }
	
	\For{$t \in \set{1,\ldots,T}$}{
	\For{$i,j\in\set{1,\ldots,N}$}{
	      $\nu^t_{i,j} \leftarrow (1-r_{i,j}^{t-1})\paran{1-\prod_{k=1}^n (1-\nu_{i,k}^{t-1} a_{k,j}\phi_k}$\;
	      $r^{t}_{i,j} \leftarrow r^{t-1}_{i,j} +(1-r_{i,j}^{t-1} )\nu^t_{i,j}$\;
	      
	}

	}
	return the matrix $R = (r^T_{i,j})_{1\leq i,j \leq N}$\;
}
\caption{\texttt{Propagate}}\label{alg:propagate}
\end{algorithm}


%Next we need to compute the vectors $(p_1,\dots, p_N)$ that minimize 
% our estimate of the cost function 
%% $$f(P_1,\dots,P_n)=\sum_{i=1}^N \frac{\pi_i}{\sum_{j=1}^N r_{i,j} P_j}.$$ 
%% and
%$$f(p_1,\dots,p_N)=\sum_{i=1}^N \frac{(1-\rho_i)\pi_i}{p_i} + \sum_{i=1}^N \frac{\rho_i \pi_i}{\sum_{j=1}^N r_{i,j}p_j}$$
%

%
%Note that if $f$ takes its minimum value at $p^* = (p^*_1, \ldots, p^*_N)$ we have the following lower bound on the optimal cost:
%$$\cost{\O} \geq \sum_{i=1}^N \frac{\pi_i}{\sum_{j=1}^N s_{i,j} p^*_j},$$
%where $\O$ is an optimal schedule.
We could compute $\mathbf{p}^*=\arg\min_{\mathbf{p}} f(\mathbf{p})$ using Lagrange multipliers, but we noticed that in practice the method of gradient descent~\cite{HastieTibshiraniFriedman201112} is more efficient and stable here.
Note that $f$ is a convex function in ${[0,1]^N}$,
and thus, $f$ is also convex on a simplex that is a convex subset of 
$[0,1]^N$:

$$\Delta^*_{N-1} = \setof{\mathbf{p}\in [0,1]^N}{\sum_i p_i = 1, \text{ and $f$ is defined at $\mathbf{p}$}}$$

Thus, every local minimum of $f$ in $\Delta^*_{N-1}$ is also a global minimum, and gradient descent is guaranteed to converge to an optimal solution.

\paragraph{Performance} Let $\mathbf{p}^*$ be the distribution $\mathbf{p}^*=\arg\min_{\mathbf{p}} f(\mathbf{p})$, and let $\R = \mathbf{p}^*$ be a randomized, memoryless 1-schedule.
% Let $\cost{\R(p^*)}$ be the cost of the randomized algorithm that uses the distribution $p^*=\arg\min_{\mathbf{p}} f(\mathbf{p})$. 
Although $\mathbf{p}^*$ optimizes a lower bound that is not tight,  
our extensive simulations with a variety of network topologies and parameters' configurations consistently show minimal difference between $\cost{\R}$ and 
$f(\mathbf{p}^*) = \min_{\mathbf{p}} f(\mathbf{p})$. To understand why $\mathbf{p}^*$ gives a near optimal schedule we need to examine the two relaxations in constructing the lower bound: (1) we assume that propagation time is negligible - this assumption is justified in our setting, where $c=o(n)$ and the graph has low diameter and/or $\rho_i <1$. In this setting the search takes significantly longer than the propagation time; (2) we use Jensen's inequality to bound a sum of exponential number of terms by an easy to compute expression. Using the notation in the proof of Theorem~\ref{thm:lower_bound_optimal_general_graph:randomized}, we bound
$g^{opt}({\mathbf{p}}) =\sum_{i=1}^N \pi_i\sum_{k=1}^{2^N} \frac{s^i_k(1-\rho_i )}{\sum_{j\in S^i_k}p_j}$  using Jensen's inequality by
$g({\mathbf{p}})= \sum_{i=1}^N \pi_i      ({\sum_{k=1}^{2^N} s^i_k \sum_{j\in S^i_k} p_j })^{-1}=
\frac{1}{\sum_{j=1}^N r_{i,j}p_ lj}$.
Our schedule is defined by 
$$\mathbf{p}^* =   \min_{\mathbf{p}}f(\mathbf{p})=  \min_{\mathbf{p}}= \paran{\sum_{i=1}^N \frac{(1-\rho_i)\pi_i}{p_i} + g({\mathbf{p})}},$$
while the optimal schedule (ignoring the propagation time) is given by
$$\mathbf{p}^{opt}
%=  \min_{\mathbf{p}}f^{opt}(\mathbf{p})
=\min_{\mathbf{p}} \paran{\sum_{i=1}^N \frac{(1-\rho_i)\pi_i}{p_i} + g^{opt}({\mathbf{p})}}.$$
Thus, $cost(\R(\mathbf{p}^*))\geq cost(\R(\mathbf{p}^{opt}))\geq f(\mathbf{p}^{opt})\geq f(\mathbf{p}^*)$, and the difference in the performance of our schedule and the optimal schedule is given by
$cost(\R(\mathbf{p}^*))- cost(\R(\mathbf{p}^{opt})) \leq g^{opt}(\mathbf{p}^*)-g(\mathbf{p}^*)$ which is the gap in applying Jensen's inequality ($\R(\mathbf{p}^*)$ and $\R(\mathbf{p}^*)$ are the randomized 1-schedules obtained from $\mathbf{p}^*$, and $\mathbf{p}^{opt}$).
% $\delta(p^*)= g^{opt}(p^*)-g(p^*)$. 
The Jensen gap is proportional to the variance in the distribution over which the expectation is taken, in particular the gap between the largest and smallest values of the random variable~\cite{Budimir2001,Cirtoaje2011}. By separating the bound into two parts, and applying the inequality only to items that were propagated at least once, we significantly limit the variation and obtain a tighter bound (details omitted for lack of space).



 % Note that $f$ and $g$ are convex functions on $[0,1]^N - \set{0}^n$:
% $$\partial^2 \frac{f}{\partial P_k \partial P_\ell}
% = \sum_{i=1}^N \frac{2\pi_i r_{i,\ell}r_{i,k}}{\paran{\sum_{j=1}^N r_{i,j}P_j}^2} > 0.
% $$
% and
% $$\partial^2 \frac{g}{\partial P_k \partial P_\ell}
% = \sum_{i=1}^N \frac{2(1-\rho_i)\pi_i}{P^2_i}+\sum_{i=1}^N \frac{2 \rho_i \pi_i r_{i,\ell}r_{i,k}}{\paran{\sum_{j=1}^N s_{i,j}P_j}^2} > 0.
% $$

% Therefore, $f$ and $g$ are also convex on the simplex $\Delta_{N-1} = \setof{p_1,\ldots,p_N}{\sum_i P_i = 1}$ which is a convex subset of 
% $[0,1]^N - \set{0}^n$, and every local minimum is also a global minimum in $\Delta_{N-1}$. We can use 
% the method of Gradient Descent that is guaranteed to find a point $P^* \in \Delta_{N-1}$ that minimizes $f$ and $g$.

%Alternatively, we can use the method of Lagrange multipliers to find an optimal solution. Let
%$$F({P},\lambda)=\sum_{i=1}^n \frac{\pi_i}{\sum_{k=1}^n r_{i,k}P_k}+\lambda(\sum_{i=1}^n P_i-1)$$
%We need all the partial derivatives with respect to the $P_j$'s to equal to 0. Thus, we have the system of equations:
%
%$$\frac{\partial F({P},\lambda)}{\partial P_j}= -\sum_{i=1}^n \frac{\pi_i r_{i,j}}{(\sum_{k=1}^n r_{i,k}P_k)^2} +\lambda =0$$ and $$\sum_{i=1}^n P_i =1.$$
%
%Using a set of auxiliary random variable:
%$$X_i =\frac{\pi_i}{(\sum_{k=1}^n r_{i,k}P_K )^2}$$
%we get a system of linear equation in $X_i,\dots, X_n$:
%$$
%\forall j \not= j  \sum_{k=1}^n X_k r_{k,j} =\sum_{k=1}^n X_k r_{k,i} .
%$$
%Let $x_1,\dots,x_n$ be a solution to the above system such that $\forall i$, $x_i>0$. We can write a second set of $n+1$ linear equations 
%in $n+1$ variables $P_i,\dots, P_n$ and $c$:
%$$\forall i~~~\sum_{k=1}^n r_{i,k}P_k= c|\sqrt{x_i\pi_i}|$$ 
%and $$\sum_{i=1}^n P_i =1.$$
%A solution to the above system gives an optimal solution.
%
%As a simple example consider a fully symmetric  case, where for all $i$, $\sum_{k=1}^n r_{k,i}=\sum_{k=1}^n r_{i,k}= d+1$.
%Note that for all $i$, $r_{i,i}=1$), and the above condition says that an item is propagated  on average to $d$ nodes, and if each node generates one item then each node receives an average of $d$ items.
%
%Clearly, in the symmetric case, $x_1=x_2,\dots,=x_n=1$ is a solution for the first system of equations, and in the solution to the second set 
%we have
%$$ c=\frac{d+1}{ \sum_{i=1}^n \sqrt{\pi_i}}.$$ 
%Plugging to the cost function we get 
%$$cost({P})=\sum_{i=1}^n \frac{\pi_i}{\sum_{k=1}^n r_{i,k}P_k}=\frac{1}{d+1} (\sum_{i=1}^n \sqrt{\pi} )^2.$$

